A Reduced-order Model for Multiphase Simulation of Transient Inert Sprays

In global efforts to reduce harmful greenhouse gas emissions from the transport sector, novel bio-hybrid liquid fuels from renewable energy and carbon sources can be a major form of energy for future propulsion systems due to their high energy density. A fundamental understanding of the spray and mixing performance of the new fuel candidates in combustion systems is necessary to design and develop the fuels for advanced combustion concepts. In the fuel design process, a large number of candidates is required to be screened to arrive at potential fuels for further detailed investigations. For such a screening process, three-dimensional (3D) simulation models are computationally too expensive and hence unfeasible. Therefore, in this paper, we present a fast, reduced-order model (ROM) for inert sprays. The model is based on the cross-sectionally averaged spray (CAS) model derived by Wan (1997) from 3D multiphase equations. The original model was first tested against a wide range of conditions and different fuels. The discrepancies between the CAS model and experimental data are addressed by integrating state-of-the-art breakup and evaporation models. A transport equation for vapor mass fraction is proposed, which is important for evaporation modeling. Furthermore, the model is extended to consider polydisperse droplets by modeling the droplet size distribution by commonly used presumed probability density functions, such as Rosin-Rammler, lognormal, and gamma distributions. The improved CAS model is capable of predicting trends in the macroscopic spray characteristics for a wide range of conditions and fuels. The computational cost of the CAS model is lower than the 3D simulation methods by up to 6 orders of magnitude depending on the method. This enables the model to be used not only for the rapid screening of novel fuel candidates, but also for other applications, where ROMs are useful.

==> figures/NewCasDSDCompare_8mm.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\definecolor{t}{rgb}{0.0,0.0,0.0}
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7936.00,5668.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1078,704){\makebox(0,0)[r]{\strut{}\color{t}$0$}}%
      \csname LTb\endcsname%%
      \put(1078,1307){\makebox(0,0)[r]{\strut{}\color{t}$20$}}%
      \csname LTb\endcsname%%
      \put(1078,1910){\makebox(0,0)[r]{\strut{}\color{t}$40$}}%
      \csname LTb\endcsname%%
      \put(1078,2513){\makebox(0,0)[r]{\strut{}\color{t}$60$}}%
      \csname LTb\endcsname%%
      \put(1078,3116){\makebox(0,0)[r]{\strut{}\color{t}$80$}}%
      \csname LTb\endcsname%%
      \put(1078,3719){\makebox(0,0)[r]{\strut{}\color{t}$100$}}%
      \csname LTb\endcsname%%
      \put(1078,4322){\makebox(0,0)[r]{\strut{}\color{t}$120$}}%
      \csname LTb\endcsname%%
      \put(1078,4925){\makebox(0,0)[r]{\strut{}\color{t}$140$}}%
      \csname LTb\endcsname%%
      \put(1210,484){\makebox(0,0){\strut{}\color{t}$0$}}%
      \csname LTb\endcsname%%
      \put(2114,484){\makebox(0,0){\strut{}\color{t}$0.005$}}%
      \csname LTb\endcsname%%
      \put(3018,484){\makebox(0,0){\strut{}\color{t}$0.01$}}%
      \csname LTb\endcsname%%
      \put(3922,484){\makebox(0,0){\strut{}\color{t}$0.015$}}%
      \csname LTb\endcsname%%
      \put(4827,484){\makebox(0,0){\strut{}\color{t}$0.02$}}%
      \csname LTb\endcsname%%
      \put(5731,484){\makebox(0,0){\strut{}\color{t}$0.025$}}%
      \csname LTb\endcsname%%
      \put(6635,484){\makebox(0,0){\strut{}\color{t}$0.03$}}%
      \csname LTb\endcsname%%
      \put(7539,484){\makebox(0,0){\strut{}\color{t}$0.035$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(462,2965){\rotatebox{-270}{\makebox(0,0){\strut{}PDF / -}}}%
      \put(4374,154){\makebox(0,0){\strut{}$d/\\Do$ / -}}%
      \put(4374,5337){\makebox(0,0){\strut{}Location: 8mm}}%
      \csname LTb\endcsname%%
      \put(6552,5054){\makebox(0,0)[r]{\strut{}LES}}%
      \csname LTb\endcsname%%
      \put(6552,4834){\makebox(0,0)[r]{\strut{}URANS}}%
      \csname LTb\endcsname%%
      \put(6552,4614){\makebox(0,0)[r]{\strut{}CAS: Rosin Rammler}}%
      \csname LTb\endcsname%%
      \put(6552,4394){\makebox(0,0)[r]{\strut{}CAS: Log Normal}}%
      \csname LTb\endcsname%%
      \put(6552,4174){\makebox(0,0)[r]{\strut{}CAS: Gamma}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/NewCasDSDCompare_8mm}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/VaporPressure.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\definecolor{t}{rgb}{0.0,0.0,0.0}
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3968.00,2834.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}0.0}}%
      \csname LTb\endcsname%%
      \put(946,1267){\makebox(0,0)[r]{\strut{}10.0}}%
      \csname LTb\endcsname%%
      \put(946,1830){\makebox(0,0)[r]{\strut{}20.0}}%
      \csname LTb\endcsname%%
      \put(946,2393){\makebox(0,0)[r]{\strut{}30.0}}%
      \csname LTb\endcsname%%
      \put(1078,484){\makebox(0,0){\strut{}300}}%
      \csname LTb\endcsname%%
      \put(1701,484){\makebox(0,0){\strut{}400}}%
      \csname LTb\endcsname%%
      \put(2325,484){\makebox(0,0){\strut{}500}}%
      \csname LTb\endcsname%%
      \put(2948,484){\makebox(0,0){\strut{}600}}%
      \csname LTb\endcsname%%
      \put(3571,484){\makebox(0,0){\strut{}700}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(330,1548){\rotatebox{-270}{\makebox(0,0){\strut{}Vapor Pressure / bar}}}%
      \put(2324,154){\makebox(0,0){\strut{}Temperature / K}}%
      \csname LTb\endcsname%%
      \put(1469,2661){\makebox(0,0)[r]{\strut{}\oct}}%
      \csname LTb\endcsname%%
      \put(2456,2661){\makebox(0,0)[r]{\strut{}\dnbe}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/./figures/VaporPressure}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> texsrc/Additional.tex <==
\begin{center}
\begin{huge}
\textbf{Additional Material} 
\end{huge}
\end{center}\\
Manuscript submitted to the International Journal of Multiphase Flow:\\
A. Y. Deshmukh, T. Grenga, M. Davidovic, L. Schumacher, J. Palmer, M. A. Reddemann, R. Kneer, H. Pitsch, A Reduced-order Model for Multiphase Simulation of Transient Inert Sprays, Int. J. Multiph. Flow (2021).



==> texsrc/highlights.tex <==
\section*{Highlights (3-5 bullet points to capture novel results )}
\begin{itemize}
\item A fast, reduced-order model based on a cross-sectionally averaged spray (CAS) is presented for transient inert sprays
\item The model prediction capability is significantly improved by the inclusion of the latest droplet breakup and evaporation models and the fuel-vapor transport
\item Trends of liquid and vapor penetrations are captured for a wide range of operating conditions and fuels
\item Information on the droplet size distribution can be obtained along the spray axis
\item Compared to 3D simulation methods, computational costs are lower by 3-6 (1-4) orders of magnitude for the monodisperse (polydisperse) CAS model
\end{itemize}
